An introduction to uncertainty quantification for kinetic equations and related problems

We overview some recent results in the field of uncertainty quantification for kinetic equations and related problems with random inputs. Uncertainties may be due to various reasons, such as lack of knowledge on the microscopic interaction details or incomplete information at the boundaries or on the initial data. These uncertainties contribute to the curse of dimensionality and the development of efficient numerical methods is a challenge. After a brief introduction on the main numerical techniques for uncertainty quantification in partial differential equations, we focus our survey on some of the recent progress on multi-fidelity methods and stochastic Galerkin methods for kinetic equations.

==> Lecture Notes NUMUQ arxiv/biblio_UQ_kinetic.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%

\begin{thebibliography}{99.}

\bibitem{albipar13}
G.~Albi, L.~Pareschi, {Binary interaction algorithms for the simulation of flocking and swarming dynamics}, {\em Multiscale Modeling \& Simulation} (2013) 11:1, 1--29 
 
\bibitem{albi2015MPE}
G.~Albi, L.~Pareschi, M.~Zanella, {Uncertainty quantification in
control problems for flocking models}, \emph{Math. Probl. Eng.}
(2015), 1--14.

%\bibitem{BS2012}
%N.~Bellomo, J.~Soler. On the mathematical theory of the dynamics of swarms viewed as complex
%systems. \emph{Mathematical Models and Methods in Applied Sciences}, 22(01): 1140006, 2012

\bibitem{AF} N.~Ayi, E.~Faou. Analysis of an asymptotic preserving scheme for stochastic linear kinetic equations in the diffusion limit. \emph{SIAM/ASA J. Uncertain. Quantif.}  7  (2019),  no. 2, 760--785.

\bibitem{BLMS} H.~Bijl, D.~Lucor, S.~Mishra, C.~Schwab (Eds.). \emph{Uncertainty Quantification in Computational Fluid Dynamics}, Lecture Notes in Computational Science and Engineering, Springer, 2013.

\bibitem{Boby} 
A.V.~Bobylev. Exact solutions of the Boltzmann equation, \emph{Dokl. Akad. Nauk SSSR}, \textbf{225}:1296--1299, 1975 (in Russian).


\bibitem{Caflisch}
R.E.~Caflisch. Monte Carlo and Quasi Monte Carlo methods. \emph{Acta Numerica}, 1-49 1998.

\bibitem{CFY} Z.~Cai, Y.~Fan, L.~Ying. 
An Entropic Fourier Method for the Boltzmann Equation. \emph{SIAM Journal on Scientific Computing} 40, (2018), A2858--A2882.


\bibitem{CPZ} {J.A.~Carrillo, L.~Pareschi, M.~Zanella}. Particle based gPC methods for mean-field models of swarming with uncertainty. \emph{Comm. Comp. Phys.} 25, 508--531, 2019.

\bibitem{CZ} {J.A.~Carrillo, M.~Zanella}. Monte Carlo gPC methods for diffusive kinetic flocking models with uncertainties. {\em Vietnam J. Math.} 47, 931--954, (2019). 

\bibitem{Cer}
C.~Cercignani. The Boltzmann Equation and its Applications. \emph{Springer--Verlag}, New York Inc., 1988. 

\bibitem{DJL} E.S.~Daus, S.~Jin, L.~Liu. Spectral convergence of the stochastic Galerkin approximation to the Boltzmann equation with multiple scales and large random perturbation in the collision kernel. \emph{Kinetic \& Related Models} 12, 909--922,(2019).


%\bibitem{CJK}
%A.~Chertock, S.~Jin, A.~Kurganov, An operator splitting based stochastic Galerkin method for the one-dimensional compressible Euler equations with uncertainty, \emph{Preprint}, 2017. 

%\bibitem{CrLe}
%N.~Crouseilles, M.~Lemou. An asymptotic preserving scheme based on a micro--macro decomposition for collisional Vlasov equation: diffusion and high--field scaling limits. \emph{Kinetic and Related Models}, 4(2): 441--477, 2011. 

\bibitem{DPe} {B.~Despr\'es, B.~Perthame}, Uncertainty propagation; Intrusive kinetic formulations of scalar conservation laws, \emph{SIAM/ASA J. Uncertainty Quantification} 4, 980--1013, 2016.

\bibitem{DPL}
B.~Despr\'es G.~Po{\"e}tte, D.~Lucor. Robust uncertainty propagation in systems of conservation laws with the entropy closure method. In \emph{Uncertainty Quantification in Computational Fluid Dynamics}, Lecture Notes in Computational Science and Engineering 92, 105--149, 2010.

\bibitem{DPR} 
P.~Degond, L.~Pareschi, G.~Russo, eds. \emph{Modeling and computational
methods for kinetic equations}, Modeling and Simulation in Science, Engineering
and Technology, Birkh\"auser Boston Inc., Boston, MA, 2004.

%\bibitem{DQP}
%G.~Dimarco, Q.~Li, B.~Yan, L.~Pareschi. Numerical methods for plasma physics in collisional regimes.\emph{ Journal of Plasma Physics:}  305810106, 2015.

%\bibitem{DLNR} G.~Dimarco, R.~Loub\'ere, J.~Narski, T.~Rey, An efficient numerical method for solving the Boltzmann equation in multidimensions, \emph{Journal of Computational Physics}, 353, 2018, pp. 46--81.

\bibitem{DPms}
G.~Dimarco, L.~Pareschi. Multi-scale control variate methods for uncertainty quantification of kinetic equations, \emph{J. Comp. Phys.} 388, 63--89, 2019.

\bibitem{DPms2}
G.~Dimarco, L.~Pareschi. Multi-scale variance reduction methods based on multiple control variates for kinetic equations with uncertainties, \emph{Mult. Mod. Sim.}, to appear.

\bibitem{DP15}
G.~Dimarco, L.~Pareschi. Numerical methods for kinetic equations. {\em Acta Numerica 23\/}, 369--520, 2014.

\bibitem{DPZ}
G.~Dimarco, L.~Pareschi, M.~Zanella. Uncertainty quantification for kinetic models in socio-economic and life sciences. {\em Uncertainty quantification for kinetic and hyperbolic equations} SEMA-SIMAI Springer Series, 2018.

\bibitem{DPZ2}
G.~Dimarco, L.~Pareschi, M.~Zanella. Micro-macro stochastic Galerkin methods for Fokker-Planck equations. Preprint 2020.

\bibitem{FDKI} H.R.~Fairbanks, A.~Doostan, C.~Ketelsen, G.~Iaccarino.
\emph{A low-rank control variate for multilevel Monte Carlo simulation of high-dimensional uncertain systems}, J. Comp. Phys., 341, 121--139, (2017).

\bibitem{GJL} I.M.~Gamba, S.~Jin, L.~Liu. Error estimate of a bi-fidelity method for kinetic equations with random parameters and multiple scales. \emph{Preprint arXiv:1910.09080}, (2019).

\bibitem{Giles}
M.B.~Giles, Multilevel Monte Carlo methods. \emph{Acta Numerica} 24, 259--328, 2015.

\bibitem{GS} C.J.~Gittelson, C.~Schwab, Sparse tensor discretization of high-dimensional parametric and stochastic PDEs, \emph{Acta Numer.}, 20 (2011), 291--467.

%\bibitem{GV} G.H.~Golub, C.F.~Van Loan. \emph{Matrix Computations} (3rd ed.), Johns Hopkins, 1996.

\bibitem{GWZ} M.D.~Gunzburger, C.G.~Webster,  G.~Zhang. Stochastic finite element methods for partial differential equations with random input data. \emph{Acta Numerica} 23, 521--650, 2014.


\bibitem{HH} J.M.~Hammersley, D.C.~Handscomb. \emph{Monte Carlo Methods.} Methuen \& Co., London, and John Wiley \& Sons, New York, 1964. 

\bibitem{HLPR} C.~Heitzinger, M.~Leum\"uller, G.~Pammer, S.~Rigger. Existence, uniqueness, and a comparison of nonintrusive methods for the stochastic nonlinear Poisson-Boltzmann equation. \emph{SIAM/ASA J. Uncertain. Quantif.}  6  (2018),  no. 3, 1019--1042.

\bibitem{HJ}
J.~Hu, S.~Jin. A stochastic Galerkin method for the Boltzmann equation with uncertainty. \emph{Journal of Computational Physics}, 315: 150--168, 2016.

\bibitem{HJS} J.~Hu, S.~Jin, R.~Shu. On stochastic Galerkin approximation of the nonlinear Boltzmann equation with uncertainty in the fluid regime, \emph{J. Comp. Phys.}, \textbf{397}, 108838, 2019

%\bibitem{JS} G.~Jiang, C.-W.~Shu. Efficient implementation of weighted ENO schemes. \emph{J. Comp. Phys.}, 126, 202--228, 1996.

%\bibitem{JinParma}
%S.~Jin. Asymptotic preserving (AP) schemes for multiscale kinetic and hyperbolic equations: a review. In \emph{ Lecture Notes for Summer School on Methods and Models of Kinetic Theory, (M\&MKT), Porto Ercole (Grosseto, Italy)}: 177-216, 2010.

\bibitem{HJS2} J.~Hu, S.~Jin, R.~Shu. A stochastic Galerkin method for the Fokker-Planck-Landau equation with random uncertainties. \emph{Theory, numerics and applications of hyperbolic problems. II}, 
 1--19, Springer Proc. Math. Stat., 237, Springer, Cham,  2018. 

\bibitem{HPW} J.~Hu, L.~Pareschi, Y.~Wang. Uncertainty quantification for the kinetic BGK equation using variance reduction multilevel Monte Carlo methods. Preprint 2020.

		 
\bibitem{JL2} S.~Jin, L.~Liu. An asymptotic-preserving stochastic Galerkin method for the semiconductor Boltzmann equation with random inputs and diffusive scalings.
 \emph{Multiscale Model. Simul.}  15  (2017),  no. 1, 157--183.

\bibitem{JinPareschi}
S.~Jin, L.~Pareschi (Eds.).  \emph{Uncertainty Quantification for Kinetic and Hyperbolic Equations}, SEMA-SIMAI Springer Series, vol. 14, Springer, 2017.

\bibitem{JPH}
S.~Jin, H.~Lu, L.~Pareschi.
Efficient Stochastic Asymptotic-Preserving Implicit-Explicit Methods for Transport Equations with Diffusive Scalings and Random Inputs, \emph{SIAM J. Sci. Comput.}, 40(2), A671--A696, 2018.

\bibitem{JPH2} S.~Jin, H.~Lu, L.~Pareschi.
A high order stochastic Asymptotic-Preserving scheme for chemotaxis kinetic models with random inputs, \emph{Mult. Model. Simul.} 6, 1884--1915, 2018.

\bibitem{JSh} S.~Jin, R.~Shu. A study of hyperbolicity of kinetic stochastic Galerkin system for the isentropic Euler equations with uncertainty. \emph{Chin. Ann. Math. Ser. B}  40  (2019),  no. 5, 765--780.
		
\bibitem{JZ}
S.~Jin, Y.~Zhu. Hypocoercivity and uniform regularity for the Vlasov-Poisson-Fokker-Planck system with uncertainty and multiple scales, \emph{SIAM J. Math. Anal.} \textbf{50}(2): 1790--1816, 2018. 

%\bibitem{LemMie}
%M.~Lemou, L.~Mieussens. A new asymptotic preserving scheme based on micro--macro %formulation for linear kinetic equations in the diffusion limit. \emph{SIAM Journal on %Scientific Computing}, 31(1): 334--368, 2008. 

\bibitem{LeMK}
O.~Le Maitre, O.M.~Knio. \emph{Spectral Methods for Uncertainty Quantification: with Applications to Computational Fluid Dynamics}, Scientific Computation, Springer Netherlands, 2010. 

\bibitem{LW} Q.~Li, L.~Wang. Uniform regularity for linear kinetic equations with random input based on hypocoercivity. \emph{SIAM/ASA J. Uncertain. Quantif.}  5  (2017),  no. 1, 1193--1219.

\bibitem{LL} L.~Liu.
A stochastic asymptotic-preserving scheme for the bipolar semiconductor Boltzmann-Poisson system with random inputs and diffusive scalings.
\emph{J. Comp. Phys.} 376, (2019), 634--659,

\bibitem {LJ} L.~Liu, S.~Jin. {Hypocoercivity based sensitivity analysis and spectral convergence of the stochastic Galerkin approximation to collisional kinetic equations with multiple scales and random inputs}, \emph{SIAM Multiscale Model. and Sim.}, 16, 1085--1114, 2018.

\bibitem{LX} L.~Liu, X.~Zhu. A bi-fidelity method for the multiscale Boltzmann equation with random parameters. {\em arXiv:1905.09023}, 2019.

\bibitem{LY}
T.-P.~Liu, S.-H.~Yu. Boltzmann equation: micro--macro decomposition and positivity of shock profiles. \emph{Communications in Mathematical Physics}, 246(1): 133--179, 2004. 

\bibitem{Lo77}
M.~Lo\`eve. \emph{Probability theory I}, 4th edition, Springer Verlag, 1977.

%\bibitem{LSV} {E.~L\o vbak, G.~Samaey, S.~Vandewalle.}
%A Multilevel Monte Carlo Asymptotic- Preserving particle method for kinetic equations in the diffusion limit, %\emph{arXiv:1902.04347}, 2019. 


\bibitem{MSS} S.~Mishra, Ch.~Schwab, J.~\v{S}ukys. Multi-level Monte Carlo finite volume methods for nonlinear systems of conservation laws in multi-dimensions. \emph{J. Comp. Phys.}, 231, 2012, 3365--3388.

\bibitem{MP} {C.~Mouhot, L.~Pareschi}. {\em Fast algorithms for computing the Boltzmann collision operator},
Math. Comp., 75, 1833--1852, 2006.

\bibitem{NPT} G.~Naldi, L.~Pareschi, G.~Toscani eds. \emph{Mathematical Modeling of Collective Behavior in Socio-Economic and Life Sciences}, Birkh{\"a}user, Boston, 2010.

\bibitem{NTW} F.~Nobile, R.~Tempone, C.G.~Webster. A sparse grid stochastic collocation method for partial differential equations with random input data. \emph{SIAM J. Num. Anal.}, 46(5):2309--2345, 2008.

\bibitem{Par2}
L.~Pareschi, G.~Russo. An introduction to Monte Carlo methods for the Boltzmann equation. \emph{ESAIM: Proceedings} \textbf{10}: 35--75, 2001.

\bibitem{Par3}
L.~Pareschi, G.~Russo. On the stability of spectral methods for the homogeneous Boltzmann equation. Transport Theory and Statistical Physics 29, (2000), 431--447.

\bibitem{PT2}
L.~Pareschi, G.~Toscani. \emph{Interacting Multiagent Systems: Kinetic Equations and Monte Carlo Methods}, Oxford University Press, 2013.  

\bibitem{PZ1}
L.~Pareschi, M.~Zanella. Structure--preserving schemes for nonlinear Fokker--Planck equations and applications. \emph{Journal of Scientific Computing}, 74, 2018, 1575--1600.

\bibitem{PZ2}
L.~Pareschi, M.~Zanella. Monte Carlo stochastic Galerkin methods for the Boltzmann equation with uncertainties: space homogeneous case. \emph{Preprint arXiv:2003.06716}, 2020.


\bibitem{PGW} B.~Peherstorfer, M.~Gunzburger, K.~Willcox. Convergence analysis of multifidelity Monte Carlo estimation. \emph{Numer. Math.} 139, 683--707, 2018. 

\bibitem{PWG} B.~Peherstorfer, K.~Willcox, M.~Gunzburger. Optimal model management for multifidelity Monte Carlo estimation. \emph{SIAM J. Sci. Comput.} 38(5), A3163?A3194, 2016.


%\bibitem{PP} B.~Perthame, M.~Pulvirenti. Weighted $L_\infty$ bounds and uniqueness for the Boltzmann BGK model, \emph{Arch. Rat. Mech. Anal.}, 125 (1993), 289--295.

\bibitem{PIN_book}
P.~Pettersson, G.~Iaccarino J.~Nordstr{\"o}m. \emph{Polynomial Chaos Methods for Hyperbolic Partial Differential Equations: Numerical Techniques for Fluid Dynamics Problems in the Presence of Uncertainties.} {Mathematical Engineering}, Springer, 2015. 

\bibitem{PDL}
G.~Po{\"e}tte, B.~Despr\'es, D.~Lucor. Uncertainty quantification for systems of conservation laws. \emph{J. Comput. Phys.}, 228(7): 2443--2467, 2009. 

%\bibitem{Rudin} W.~Rudin. {\em Real and Complex Analysis}. Mladinska Knjiga, McGraw-Hill, 1970.

\bibitem{Po} 
G. Po\"ette. 
A gPC-intrusive Monte-Carlo scheme for the resolution of the uncertain linear Boltzmann equation,
\emph{J. Comput. Phys.} {385}, 135--162, 2019.

\bibitem{Po2} 
G. Po\"ette. Spectral convergence of the generalized Polynomial Chaos reduced model obtained from the uncertain linear Boltzmann equation.  \emph{Preprint hal-02090593v2}, (2020).


\bibitem{RKA}
F.~Roosta-Khorasani, K.~van den Doel, U.~Ascher. Stochastic Algorithms for Inverse Problems Involving PDEs and many Measurements. {\em SIAM J. Sci. Comput.}, 36(5), S3–S22. (2014).

\bibitem{RSS} G.~Russo, P.~Santagati, S-B.~Yun. Convergence of a Semi-Lagrangian Scheme for the BGK Model of the Boltzmann Equation. \emph{SIAM J. Numer. Anal.}, 50(3), (2012), 1111--1135. 

\bibitem{RHS} R.~Shu, J.~Hu, S.~Jin, A Stochastic Galerkin Method for the Boltzmann Equation with multi-dimensional random inputs using sparse wavelet bases, \emph{Num. Math.: Theory, Methods and Applications (NMTMA)}, 10, 465--488, 2017. 

%\bibitem{Son} E.~Sonnendrucker. \emph{Numerical methods for Vlasov equations}. {Technical report}, MPI TU
%Munich, 2013.

\bibitem{Tos1999}
G.~Toscani. Entropy production and the rate of convergence to equilibrium for the Fokker--Planck equation. \emph{Quarterly of Applied Mathematics}, LVII(3): 521--541, 1999. 

\bibitem{ToVil}
G.~Toscani, C.~Villani. Sharp entropy dissipation bounds and explicit rate of trend to equilibrium for the spatially homogeneous Boltzmann equation. \emph{Communications in Mathematical Physics}, 203(3): 667--706, 1999. 

%\bibitem{Trist}
%I.~Tristani. Exponential Convergence to Equilibrium for the Homogeneous Boltzmann Equation for Hard Potentials Without Cut-Off. \emph{Journal of Statistical Physics}, 157(3): 474--496, 2014.

\bibitem{Vill}
C.~Villani. A review of mathematical topics in collisional kinetic theory. In S. Friedlander, D. Serre Eds. \emph{Handbook of Mathematical Fluid Mechanics}, Vol. I, p.71--305, North--Holland, 2002.

%\bibitem{Vlas}
%A.A.~Vlasov. \emph{Many--Particle Theory and its Application to Plasma}. Russian Monographs and Text on Advanced Mathematics and Physics, Vol. VII. {Gordon and Breach, Science Publishers, Inc.}, New York, 1961.

\bibitem{Xu}
D.~Xiu. \emph{Numerical Methods for Stochastic Computations}. {Princeton University Press}, 2010.

\bibitem{ZJ} Y.~Zhu, S.~Jin, The Vlasov-Poisson-Fokker-Planck system with uncertainty and a one-dimensional asymptotic-preserving method , \emph{SIAM Multiscale Model. Simul.}, 15(4), 1502--1529, 2017.

\bibitem{ZLX} X.~Zhu, E.M.~Linebarger, D.~Xiu, Multi-fidelity stochastic collocation method for computation of statistical moments, \emph{J. Comput. Phys.}, 341, 386--396, 2017.

\end{thebibliography}


